Chain of Execution Supervision Promotes General Reasoning in Large Language Models

Building robust and general reasoning ability is a central goal in the development of large language models (LLMs). Recent efforts increasingly turn to code as a rich training source, given its inherent logical structure and diverse reasoning paradigms such as divide-and-conquer, topological ordering, and enumeration. However, reasoning in code is often expressed implicitly and entangled with syntactic or implementation noise, making direct training on raw code suboptimal.To address this, we introduce TracePile, a large-scale corpus of 2.6 million samples that transforms code execution into explicit, step-by-step chain-of-thought-style rationales, which we call Chain of Execution (CoE). The corpus spans domains including mathematics, classical algorithms and algorithmic competition, and is enriched with variable-tracing questions and code rewritings to enhance logical granularity and code diversity. We evaluate TracePile using three training setups: continue-pretraining, instruction tuning after pretraining, and two-stage finetuning. Experiments across four base models (LLaMA 3, LLaMA 3.1, Qwen-2.5, and Qwen-2.5 Coder) and 20 benchmarks covering math, code, logic, and algorithms demonstrate consistent improvements. Notably, TracePile boosts LLaMA3.1-8B by 7.1\% on average across nine math datasets and delivers clear gains on LiveCodeBench, CRUX, and MMLU under two-stage fine-tuning.

==> Tables/main_results.tex <==
\begin{table*}[h!]

\centering
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1.3} % 增大行距
\resizebox{\textwidth}{!}{%
\huge % 增大字体
\definecolor{custompurple}{RGB}{208,224,239}
\begin{tabular}{l|ccccccccccc|c}
\toprule

\multicolumn{13}{c}{\textbf{Two Stage Instruction Tuning}} \\ \midrule
& \multicolumn{11}{c|}{\textbf{Mathematical Reasoning}} \\ \midrule
\textbf{Models} & \textbf{GSM8K} & \textbf{MinMath} & \textbf{MATH} & \textbf{GSM-Hard} & \textbf{SVAMP} & \textbf{ASDIV} & \textbf{MAWPS} & \textbf{STEM} & \textbf{TABMWP} & \textbf{MATHQA} & \textbf{SAT} & \underline{\textbf{Avg.}}\\ 
\midrule

Llama-3-8b  & 70.70 & 28.80 & 28.60 & 35.00 & 83.00 & 81.40 & 93.90 & 42.80 & 65.80 & 37.70 & 40.60 & 55.30\\
\multicolumn{1}{r|}{+ \ourdataset}       &  74.00 & 33.80 & 30.60 & 35.60 & 79.40 & 81.90 & 93.50 & 52.90 & 67.10 & 54.70 & 75.00 & 61.70 \\ \midrule
Llama-3.1-8b               & 54.4 & 20.4 & 17.7 & 27.1 & 71.0 & 74.3 & 92.0 & \cellcolor{custompurple}\textbf{57.0} & \cellcolor{custompurple}\textbf{63.6 }& 44.9 &59.4 &52.9\\
\multicolumn{1}{r|}{+ \ourdataset}      & \cellcolor{custompurple}\textbf{66.0} & \cellcolor{custompurple}\textbf{23.6} & \cellcolor{custompurple}\textbf{24.1} & \cellcolor{custompurple}\textbf{30.9} & \cellcolor{custompurple}\textbf{78.4} & \cellcolor{custompurple}\textbf{79.6} & \cellcolor{custompurple}\textbf{92.0} & 56.4 & 59.2 & \cellcolor{custompurple}\textbf{53.1} & \cellcolor{custompurple}\textbf{59.4} &\cellcolor{custompurple}\textbf{56.6} \\ 

Qwen-2.5-7b      & 26.9 & 14.4 & 13.2 & 16.8 & 48.7 & 62.3 & 77.6 & \cellcolor{custompurple}\textbf{43.6} & 39.6 & 32.8 & \cellcolor{custompurple}\textbf{53.1} &39.0 \\
\multicolumn{1}{r|}{+ \ourdataset} & \cellcolor{custompurple}\textbf{36.8} & \cellcolor{custompurple}\textbf{15.0} & \cellcolor{custompurple}\textbf{18.7 }& \cellcolor{custompurple}\textbf{18.5} & \cellcolor{custompurple}\textbf{58.6} &\cellcolor{custompurple}\textbf{66.0} & \cellcolor{custompurple}\textbf{83.9} & 41.9 & \cellcolor{custompurple}\textbf{42.0} & \cellcolor{custompurple}\textbf{38.0} & 40.6 &\cellcolor{custompurple}\textbf{41.8} \\
\midrule


Qwen-2.5-7b-coder      & 26.9 & 14.4 & 13.2 & 16.8 & 48.7 & 62.3 & 77.6 & \cellcolor{custompurple}\textbf{43.6} & 39.6 & 32.8 & \cellcolor{custompurple}\textbf{53.1} &39.0 \\
\multicolumn{1}{r|}{+ \ourdataset} & \cellcolor{custompurple}\textbf{36.8} & \cellcolor{custompurple}\textbf{15.0} & \cellcolor{custompurple}\textbf{18.7}& \cellcolor{custompurple}\textbf{18.5} & \cellcolor{custompurple}\textbf{58.6} &\cellcolor{custompurple}\textbf{66.0} & \cellcolor{custompurple}\textbf{83.9} & 41.9 & \cellcolor{custompurple}\textbf{42.0} & \cellcolor{custompurple}\textbf{38.0} & 40.6 &\cellcolor{custompurple}\textbf{41.8} \\
\midrule






\bottomrule

\end{tabular}
}
\vspace{0.5cm} % Add space between the two tables

\resizebox{\textwidth}{!}{%
% \huge % 增大字体
\definecolor{custompurple}{RGB}{208,224,239}
\begin{tabular}{l|ccc|cc|cc|cc|c} % 删除了 Avg. 列
\toprule
                           & \multicolumn{3}{c|}{\textbf{Logical Reasoning}} & \multicolumn{2}{c|}{\textbf{Commonsense Reasoning}} & \multicolumn{2}{c|}{\textbf{Code Reasoning}} & \multicolumn{2}{c|}{\textbf{Graph Problem Reasoning}} &  \\ \midrule
 \textbf{Models}       & \textbf{Zebra Puzzles}              & \textbf{Ruletaker}       & \textbf{ProofWriter}   & \textbf{StrategyQA}  & \textbf{Hellaswag} &\textbf{LCB}     &\textbf{ CLRS } & \textbf{GraphWiz} & \textbf{GraphInstruct} &\underline{\textbf{Avg.}}\\ 
\midrule
Llama-3-8b         &10.0                                  & 22.8                           & 25.0    &66.2 &48.3       & 2.9      & 3.3          & 4.5       & 35.2 &24.2       \\
\multicolumn{1}{r|}{+ \ourdataset}    &\cellcolor{custompurple}\textbf{24.0 }                    & \cellcolor{custompurple}\textbf{43.1} &  \cellcolor{custompurple}\textbf{41.6}   &\cellcolor{custompurple}\textbf{69.7} &\cellcolor{custompurple}\textbf{52.8}       & \cellcolor{custompurple}\textbf{6.9 } & \cellcolor{custompurple}\textbf{49.9}      & \cellcolor{custompurple}\textbf{49.9} &\cellcolor{custompurple}\textbf{70.8} &\cellcolor{custompurple}\textbf{45.4}       \\
\midrule
Llama-3.1-8b                     &18.0                   & 35.3                          & 29.8    &58.9 &48.7         & 1.6  & 3.3     & 1.9       & 33.0 & 25.8        \\
\multicolumn{1}{r|}{+ \ourdataset}        &\cellcolor{custompurple}\textbf{34.0 }               & \cellcolor{custompurple}\textbf{61.1}                        & \cellcolor{custompurple}\textbf{40.9}    &\cellcolor{custompurple}\textbf{69.6} &\cellcolor{custompurple}\textbf{53.6}     &  \cellcolor{custompurple}\textbf{12.5}   &  \cellcolor{custompurple}\textbf{5.6 }        & \cellcolor{custompurple}\textbf{52.2}      & \cellcolor{custompurple}\textbf{74.9} & \cellcolor{custompurple}\textbf{44.9 }       \\  
\midrule
Qwen-2.5-7b                     &18.0                   & 35.3                          & 29.8    &58.9 &48.7         & 1.6  & 3.3     & 1.9       & 33.0 & 25.8        \\
\multicolumn{1}{r|}{+ \ourdataset}        &\cellcolor{custompurple}\textbf{34.0 }               & \cellcolor{custompurple}\textbf{61.1}                        & \cellcolor{custompurple}\textbf{40.9}    &\cellcolor{custompurple}\textbf{69.6} &\cellcolor{custompurple}\textbf{53.6}     &  \cellcolor{custompurple}\textbf{12.5}   &  \cellcolor{custompurple}\textbf{5.6 }        & \cellcolor{custompurple}\textbf{52.2}      & \cellcolor{custompurple}\textbf{74.9} & \cellcolor{custompurple}\textbf{44.9 }       \\  
\midrule
Qwen-2.5-7b-Coder                     &18.0                   & 35.3                          & 29.8    &58.9 &48.7         & 1.6  & 3.3     & 1.9       & 33.0 & 25.8        \\
\multicolumn{1}{r|}{+ \ourdataset}        &\cellcolor{custompurple}\textbf{34.0 }               & \cellcolor{custompurple}\textbf{61.1}                        & \cellcolor{custompurple}\textbf{40.9}    &\cellcolor{custompurple}\textbf{69.6} &\cellcolor{custompurple}\textbf{53.6}     &  \cellcolor{custompurple}\textbf{12.5}   &  \cellcolor{custompurple}\textbf{5.6 }        & \cellcolor{custompurple}\textbf{52.2}      & \cellcolor{custompurple}\textbf{74.9} & \cellcolor{custompurple}\textbf{44.9 }       \\  
\bottomrule
\end{tabular}
}
\caption{Main results on mathematical benchmarks (top) and other benchmarks (bottom), where LCB represents Livecodebench.}

% \vspace{-0.4cm}
\label{tab:main_table}
\end{table*}

==> Tables/main_results_cpt_algined.tex <==
%%% Preamble (add or merge with existing) %%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}[h]  % fixed bracket
\centering
\caption{Model performances under continue-pretraining. L.C.Bench-O refers to the test-output subset of LiveCodeBench.}
\renewcommand{\arraystretch}{1.1}
\label{continue pretrain}
\resizebox{\textwidth}{!}{%
\begin{tabular}{
  c|c|
  S[table-format=3.1] S[table-format=3.1]|
  S[table-format=3.1] S[table-format=3.1]|
  S[table-format=3.1] S[table-format=3.1]|
  S[table-format=3.1] S[table-format=3.1]
}
\toprule
\multirow{2}{*}{\textbf{Type}} &
  \multirow{2}{*}{\textbf{Datasets}} &
  \multicolumn{2}{c|}{\textbf{Llama-3-8B}} &
  \multicolumn{2}{c|}{\textbf{Llama-3.1-8B}} &
  \multicolumn{2}{c|}{\textbf{Qwen-2.5-7B}} &
  \multicolumn{2}{c}{\textbf{Qwen-2.5-Coder}} \\
\cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10}
&
& \multicolumn{1}{c}{Base} & \multicolumn{1}{c|}{Ours}
& \multicolumn{1}{c}{Base} & \multicolumn{1}{c|}{Ours}
& \multicolumn{1}{c}{Base} & \multicolumn{1}{c|}{Ours}
& \multicolumn{1}{c}{Base} & \multicolumn{1}{c}{Ours} \\
\midrule
\multirow{10}{*}{Math}
& GSM8K        & 54.2 & \best{\textbf{74.3}} & 54.4 & \best{\textbf{74.7}} & \best{\textbf{85.7}} & 84.9 & 77.9 & \best{\textbf{83.5}} \\
& MATH         & 16.5 & \best{\textbf{31.7}} & 17.7 & \best{\textbf{29.3}} & \best{\textbf{50.9}} & 44.8 & 47.2 & \best{\textbf{52.3}} \\
& GSM-H        & 26.1 & \best{\textbf{36.2}} & 27.1 & \best{\textbf{36.9}} & \best{\textbf{63.3}} & 63.1 & 55.1 & \best{\textbf{59.8}} \\
& SVAMP        & 68.8 & \best{\textbf{81.2}} & 71.0 & \best{\textbf{81.1}} & 89.4 & \best{\textbf{89.6}} & 87.8 & \best{\textbf{89.0}} \\
& ASDIV        & 73.1 & \best{\textbf{82.7}} & 74.3 & \best{\textbf{83.8}} & 91.0 & \best{\textbf{91.3}} & 89.0 & \best{\textbf{89.2}} \\
& MAWPS        & 90.9 & \best{\textbf{92.2}} & 92.0 & \best{\textbf{93.7}} & 97.0 & \best{\textbf{97.1}} & 93.5 & \best{\textbf{94.9}} \\
& STEM         & 49.7 & \best{\textbf{56.3}} & 57.0 & \best{\textbf{57.1}} & 68.0 & \best{\textbf{72.6}} & 67.2 & \best{\textbf{68.3}} \\
& TABMWP       & 57.9 & \best{\textbf{55.0}} & \best{\textbf{63.6}} & 57.4 & \best{\textbf{73.0}} & 72.3 & 56.9 & \best{\textbf{66.2}} \\
& SAT          & 56.2 & \best{\textbf{53.1}} & 59.4 & \best{\textbf{68.8}} & 80.0 & \best{\textbf{93.8}} & 81.2 & \best{\textbf{84.4}} \\
\cmidrule{2-10}
& Average      & 54.8 & \best{\textbf{62.5}} & 57.4 & \best{\textbf{64.8}} & 77.6 & \best{\textbf{78.8}} & 72.9 & \best{\textbf{76.4}} \\
\midrule
\multirow{1}{*}{Code}
& L.C.Bench-O  &  2.0 & \best{\textbf{30.5}} &  1.6 & \best{\textbf{11.8}} & 40.3 & \best{\textbf{49.8}} & 14.0 & \best{\textbf{44.8}} \\
\midrule
\multirow{3}{*}{Logical}
& Zebra Puzzle &  0.1 & \best{\textbf{ 7.4}} &  2.3 & \best{\textbf{ 7.4}} & \best{\textbf{ 2.9}} &  2.0 &  3.0 & \best{\textbf{ 4.0}} \\
& KORBench &\best{\textbf{21.8}}& \best{\textbf{21.8}} & \best{\textbf{21.9}} & 20.6 & 33.4 & \best{\textbf{35.4}} & \best{\textbf{32.0}} & 30.0 \\
& Ruletaker    &  2.8 & \best{\textbf{42.4}} &  5.3 & \best{\textbf{45.6}} & 61.2 & \best{\textbf{63.5}} & 46.1 & \best{\textbf{60.2}} \\
\midrule
\multirow{2}{*}{Algorithm}
& Graphwiz     &  4.5 & \best{\textbf{46.0}} &  1.9 & \best{\textbf{33.9}} & 36.6 & \best{\textbf{50.5}} & 38.5 & \best{\textbf{43.8}} \\
& GraphInstruct& 35.2 & \best{\textbf{73.5}} & 33.0 & \best{\textbf{69.2}} & 33.1 & \best{\textbf{33.5}} & 33.8 & \best{\textbf{53.7}} \\
\bottomrule
\end{tabular}}
\end{table}

